Belief propagation in monoidal categories

We discuss a categorical version of the celebrated belief propagation algorithm. This provides a way to prove that some algorithms which are known or suspected to be analogous, are actually identical when formulated generically. It also highlights the computational point of view in monoidal categories.

==> eptcsdata.tex <==
\providecommand{\firstpage}{262}
\providecommand{\publicationstatus}{B. Coecke, I. Hasuo \& P. Panangaden (Eds.):\\
Quantum Physics and Logic 2014 (QPL 2014).\\
EPTCS 172, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.172.18}{10.4204/EPTCS.172.18}}

